BOMP: Bin-Optimized Motion Planning

In logistics, the ability to quickly compute and execute pick-and-place motions from bins is critical to increasing productivity. We present Bin-Optimized Motion Planning (BOMP), a motion planning framework that plans arm motions for a six-axis industrial robot with a long-nosed suction tool to remove boxes from deep bins. BOMP considers robot arm kinematics, actuation limits, the dimensions of a grasped box, and a varying height map of a bin environment to rapidly generate time-optimized, jerk-limited, and collision-free trajectories. The optimization is warm-started using a deep neural network trained offline in simulation with 25,000 scenes and corresponding trajectories. Experiments with 96 simulated and 15 physical environments suggest that BOMP generates collision-free trajectories that are up to 58 % faster than baseline sampling-based planners and up to 36 % faster than an industry-standard Up-Over-Down algorithm, which has an extremely low 15 % success rate in this context. BOMP also generates jerk-limited trajectories while baselines do not. Website: https://sites.google.com/berkeley.edu/bomp.

==> 6-limitations.tex <==
\section{Limitations}\label{limitations}

% \paragraph*{\bf Grasped Object Depth Estimation}
% Due to occlusions, it is often impossible to tell the depth of an object. In this work, we get around this problem by \zach{ethan what is the strategy?}. However, any heuristic tries to balance between having fast trajectories (by keeping capsule size minimal) and not colliding (by keeping capsule size adequately large).

\paragraph*{\bf Capsule Carving}
\zach{I would be okay to cut this section since it is a lukewarm issue at best}
Capsule carving (\ref{carving}) effectively solves the problem of collision with the environment at the beginning of our trajectory. However, this method may cause unintended side effects. Since the capsule model overestimates the actual volume of the box, it tends to carve into adjacent obstacles. As a result, the motion planner may compute a solution that would collide in real since not all of the collision environment is present in the carved depth map it uses to plan. % wait this section is unused -- going to add this to the discussion of limitations in 7-discussion ok

This issue is especially apparent if a box is positioned sufficiently near the edge of a bin. In this case, parts of the bin walls could be carved out, resulting in potential collisions with the bin walls.
% the capsule created for that box would have the spherical parts extend through the walls.
% When we perform carving in this setting, the walls of the bin will also be removed since they are in collision with the capsule.
% However, due to the tightness of the carve relative to the capsule size, the capsule should never be able to fully pass through the generated gap as the diameter will be part of the box and not cut through the bin wall. \zach{this probably needs to be explained better, but basically the idea is that the hole in the wall will never be cut by the widest part of the capsule because the widest part of the capsule is the middle/diagonal of the box, which can't be through the bin wall otherwise the box would already be inside the wall}
% \input{figures/filler}

\paragraph*{\bf Very Large Capsules}
\label{large_capsules}
When the grasped object is exceedingly large (i.e., more than about 20cm in the biggest side), modeling it with a single capsule becomes a very poor approximation. For safety, the capsule must fully circumscribe the box it models. However, the tightest such capsule fully contains the box within its cylindrical section.

The radius of a capsule is computed as $\sqrt{a^2+b^2}$ where $a, b$ are the smallest two sides of the box. When the radius is large, the two hemi-spheres at the ends of the capsule take up more volume, with cubic scaling. As a result, planned trajectories become convoluted and suboptimal, or even impossible altogether \zach{reference the impossible cases here}. Furthermore, for these large capsules, an unrealistic amount of the depth map is removed in the carving process (\ref{carving}). In future work, we hope to solve this problem by modeling each object with a set of multiple capsules. However, this massively increases the computation time due to the increased number of capsule-capsule collisions to be checked (number of robot capsules $\times$ depth map width $\times$ depth map height). \zach{this product should probably be formalized somewhere}
% In future work \zach{actually probably in the revision}, we hope to solve this problem by subdividing the cube, and modeling the grasped object as a set of neighboring capsules of some maximum radius, packed together as in a pack of hot dogs.

==> figures/old/figure_two.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=1.0\linewidth]{figures/raw_images/sim_complete.png}
\caption{
Simulation setup at initialization (7 layers)
}
\label{fig:figure_two}
\end{figure}


==> figures/old/filler.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=1.0\linewidth]{figures/raw_images/filler_graph.jpg}
\caption{
\ethan{TODO: replace with actual graph}
}
\label{fig:filler figure}
\end{figure}


==> figures/old/physical.tex <==
\begin{table}[h]
\vspace{6pt}
% \rule{0pt}{2pt}\\
    \caption{Physical experiment results. MPT is run over 5 trajectories and the mean (min, max) are reported. The number (1 or 10) is the number of seconds given for max solve time. Additional time is due to trajectory parameterization from waypoints. A success is considered if a collision-free trajectory is generated. In the MPT-1 failure case in scene 2, the wrist of the robot collides with the camera stand (as collisions are not checked with the links of the robot). }
\begin{adjustbox}{width=\columnwidth,center}
    \centering
\begin{tabular}{c c c c c}
    \hline
    Algorithm&Computation Success Rate&Compute Time (s)&Execution Time (s) & Execution Success Rate\\
    \hline
    \hline
%   \multirow{3}*{1}&Up and Over&Y&N/A&$5.8$\\
% &GOMP-EDGE&Y&&$0.8$\\ 
%     \hline
%   \multirow{3}*{2}&Up and Over&Y&N/A&5.5\\
% &GOMP-EDGE&Y&&2.0\\ 
% \hline
%   \multirow{3}*{3}&Up and Over&Y&N/A&5.0\\
% &GOMP-EDGE&Y&&1.2\\ 
% \hline
%   \multirow{3}*{4}&Up and Over&Y&N/A&5.6\\
% &GOMP-EDGE&Y&&\\ 
% \hline
%   \multirow{3}*{5}&Up and Over&Y&N/A&?\\
% &GOMP-EDGE&Y&&\\ 
    GOMP-EDGE & & & & \\
    \hline
    MPT-1 & & & & \\
    \hline
    MPT-10 & 100\%* & & & \\
    \hline
    Up-Over-Down & & & & \\
    \hline
    GOMP-EDGE(-OH) & & & & \\
    \hline
    GOMP-EDGE-COLD & & & & \\
\hline
\end{tabular}
%     \centering
% \begin{tabular}{c c c c c}
%     \hline
%     Scene&Algorithm&Success&Compute (s) &Execution (s) \\
%     \hline
%     \hline
%   \multirow{3}*{1}&&&&\\
% &MPT-1&&&\\ 
% &MPT-10&&&\\ 
% &GOMP-EDGE&&&\\ 
%     \hline
%   \multirow{3}*{2}&Up and Over&&&\\
% &MPT-1&&&\\ 
% &MPT-10&&&\\ 
% &GOMP-EDGE&&&\\ 
% \hline
%   \multirow{3}*{3}&Up and Over&&&\\
% &MPT-1&&&\\ 
% &MPT-10&&&\\ 
% &GOMP-EDGE&&&\\ 
% \hline
%   \multirow{3}*{4}&Up and Over&&&\\
% &MPT-1&&&\\ 
% &MPT-10&&&\\ 
% &GOMP-EDGE&&&\\ 
% \hline
%   \multirow{3}*{5}&Up and Over&&&\\
% &MPT-1&&&\\ 
% &MPT-10&&&\\ 
% &GOMP-EDGE&&&\\ 
% \hline
% \end{tabular}

\label{tab:phy_result}
\end{adjustbox}

\end{table}


==> figures/physical_setup.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figures/raw_images/new_workspace.png}
\caption{\textbf{Workcell for physical environments}. In our experiments, we consider a UR5 robot picking a box from a large bin filled with boxes of assorted sizes.  \AlgName{} and baselines compute motions to move the grasped object to a collision-free end point outside the bin. Before each motion, an overhead camera captures an RGBD image of the bin.  The long suction end effector attached to the robot allows it to reach deep into the bin.
% \karthik{TODO trim, fill in mock up boxes}
}
\label{fig:workcell}
\end{figure}

